Applying Distributional Compositional Categorical Models of Meaning to Language Translation

The aim of this paper is twofold: first we will use vector space distributional compositional categorical models of meaning to compare the meaning of sentences in Irish and in English (and thus ascertain when a sentence is the translation of another sentence) using the cosine similarity score. Then we shall outline a procedure which translates nouns by understanding their context, using a conceptual space model of cognition. We shall use metrics on the category ConvexRel to determine the distance between concepts (and determine when a noun is the translation of another noun). This paper will focus on applications to Irish, a member of the Gaelic family of languages.

==> eptcsdata.tex <==
\providecommand{\firstpage}{28}
\providecommand{\publicationstatus}{B. Coecke, J. Hedges, D. Kartsaklis, M. Lewis, D. Marsden (Eds.):\\2018 Workshop on Compositional Approaches\\for Physics, NLP, and Social Sciences (CAPNS)\\
EPTCS 283, 2018, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.283.3}{10.4204/EPTCS.283.3}}

